Don't Pick the Cherry: An Evaluation Methodology for Android Malware Detection Methods

In evaluating detection methods, the malware research community relies on scan results obtained from online platforms such as VirusTotal. Nevertheless, given the lack of standards on how to interpret the obtained data to label apps, researchers hinge on their intuitions and adopt different labeling schemes. The dynamicity of VirusTotal's results along with adoption of different labeling schemes significantly affect the accuracies achieved by any given detection method even on the same dataset, which gives subjective views on the method's performance and hinders the comparison of different malware detection techniques. In this paper, we demonstrate the effect of varying (1) time, (2) labeling schemes, and (3) attack scenarios on the performance of an ensemble of Android repackaged malware detection methods, called dejavu, using over 30,000 real-world Android apps. Our results vividly show the impact of varying the aforementioned 3 dimensions on dejavu's performance. With such results, we encourage the adoption of a standard methodology that takes into account those 3 dimensions in evaluating newly-devised methods to detect Android (repackaged) malware.

==> parts/2motivation.tex <==
\section{Motivating Example}
\label{sec:motivation}
In this section, we motivate the need for our paper and its line of research via an example. 
As part of the Android malware analysis and detection research community, we devise and evaluate new methods to help counter its spread. 
During our evaluation of \dejavu's components, particularly the \emph{quick matching} module, against the \emph{Piggybacking} dataset we came across different dubious scenarios.
In summary, the \emph{quick matching} module attempts to utilize compiler fingerprinting to classify apps as malicious or benign. 
That is, if two apps, one of which is a reference app presumed to be benign, match in terms of package name, description, and other metadata but have different codebases (i.e., in terms of the \texttt{classes.dex} file), the module attempts to fingerprint the compilers used to compile their APK archives. 
According to the fingerprinted compilers of both apps, the module decides, in a manner we thoroughly discuss in section \ref{sec:dejavu}, upon whether the app we are checking (i.e., test app), is a repackaged, malicious version of the reference app. 

One of the scenarios we encountered was during testing an app called \texttt{TP.LoanCalculator}. 
Despite being labeled by the authors of the \emph{Piggybacking} dataset as malicious, the \emph{quick matching} module deemed the test app\footnote{2b44135f245a2bd104c4b50dc9df889dbd8bc79b} as benign. 
After inspection, we found that the module classified the aforementioned test app as benign because it matched a reference app\footnote{d8472cf8dcc98bc124bd5144bb2689785e245d83} in terms of metadata, used compiler, and even codebase. 
Consequently, the quick matching module considered the test app as yet another version of the benign reference app. 

Given that the dataset comprises benign apps and their repackaged malicious versions, it is expected to find apps that match in terms of metadata, graphical user interface, and file names. 
However, two apps possessing the exact same codebase implies that they are basically the same apps, perhaps with slight modifications to their resource files (e.g., strings and colors), or certificates.
So, how can two apps with identical metadata and codebases be simultaneously deemed as malicious and benign.
One possible answer to this question is that one of the apps added malicious code to one of the resource files (e.g., to be loaded and executed during runtime). 
However, the added code needs to be loaded by some app component, which requires modifying the original codebase leading to two two different codebases. 
The more plausible answer is that either, or both, apps were given incorrect labels. 
In \cite{li2017understanding}, the authors of the \emph{Piggybacking} dataset labeled the apps they gathered with the aid of \texttt{VirusTotal} scan results. 
An app was labeled as malicious if at least one scanner deemed it as malicious and was labeled as benign otherwise.

In this context, we retrieved the \texttt{VirusTotal} results of both app versions. 
On the one hand, the test app was labeled malicious by 14 out of 60 antiviral software scanners. 
We noticed, however, that the results acquired from \texttt{VirusTotal} indicated that the app was first analyzed in 2013. 
So, we uploaded the app's APK archive for re-analysis in late 2018 to see whether the number of scanners would differ. 
The 2018 version of the scan results indicated that three more scanners deemed the app malicious. 

On the other hand, the scan results obtained for the reference app were more interesting. 
Similar to its malicious version, this presumeably benign app was first scanned in 2013. 
In this case, the scan results from \texttt{VirusTotal} indicated that all scanners deemed the app as benign, displaying green \textbf{Clean} labels next to all scanners.
Nevertheless, after clicking on the \emph{Reanalyze} button, 17 of the green labels turned red displaying different malware family names that indicate the malignance of the app.
That is to say, the reference app originally labeled and released as part of the \emph{Piggybacking} dataset as a benign app is, in fact, another version of a malicious app of the type \texttt{Adware}. 

Needless to say, the authors of the \emph{Piggybacking} did not intentionally mislabel apps. 
The most likely scenario is that, at the time of releasing the dataset, the reference app was still deemed as benign by the \texttt{VirusTotal} scanners.
Our example shows the evolution of scan results returned by \texttt{VirusTotal} and the impact of time on them. 
This phenomenon implies that prior to using any dataset--including manually-labeled ones, all apps need to be re-analyzed and re-labeled. 
Having mentioned labeling, our example shows that 17 out of 60 scanners (i.e., 28.33\%), deemed both apps as malicious. 
Interestingly, some renowned scanners including AVG, McAfee, Kaspersky, Microsoft, and TrendMicro continue to deem both apps as benign. 
However, according to the authors' criterion to label an app as malicious if at least \textbf{one} scanner deems it so, both apps would be labeled as malicious.
The same would not hold for the authors of the \emph{AMD} dataset who consider an app as malicious if at least 50\% (out of 55) of the \texttt{VirusTotal} scanners deem it malicious. 
Those two dimensions (i.e., time and labeling scheme/criteria), are expected to affect the performance of any detection framework using the same dataset, especially if the malicious apps are repackaged or belong to an ambiguous malware type such as \texttt{Adware} or \texttt{Riskware}.
This paper attempts to demonstrate the effect of varying those two dimensions on the performance of an ensemble method, \dejavu, built to detect Android repackaged malware. 
%\textcolor{red}{more experiments to demonstrate time effect? We have results from CODASPY!}







